One Call Ahead: Packed Self-Speculative Decoding with Diffusion Drafting

Autoregressive (AR) language models generate tokens sequentially, so generating long outputs is costly. Speculative decoding mitigates this by using a lightweight drafter to propose multiple tokens for the target AR model to verify in parallel, while a diffusion-based drafter can produce an entire draft block in one forward pass. In models with AR and diffusion modes, one network both drafts and verifies, but drafting still waits for verification, so the standard schedule needs two sequential model calls per iteration. Existing one-call schedules avoid the wait but incur input size quadratic in the speculative width. Motivated by this efficiency bottleneck, we introduce Packed-SS, a self-speculative decoding schedule that verifies and drafts in a single model call with input size linear in the speculative width, while preserving the target model's distribution. The key idea is to let the diffusion drafter run one call ahead: while verifying the current draft, the model simultaneously constructs the next draft from an older verified prefix and keeps its unresolved suffix for the next iteration. Under a mild monotonicity assumption on the drafter, we further show that Packed-SS requires no more model calls than the standard two-call decoding in the greedy setting. Experiments on Nemotron 3B/8B and SetDLM 1.7B show higher throughput and lower mean wall time than both baselines under greedy decoding.

==> figures/efficiency_style.tex <==
\newcommand{\efficiencyPanelFont}{\fontsize{8}{9}\selectfont\bfseries}
\newcommand{\efficiencyGroupFont}{\fontsize{7}{8}\selectfont\bfseries}
\newcommand{\efficiencyTaskFont}{\fontsize{7}{8}\selectfont}
\newcommand{\efficiencyTickFont}{\fontsize{6}{7}\selectfont}
\newcommand{\efficiencyLegendFont}{\fontsize{9}{10}\selectfont}

\pgfplotsset{
  efficiency axis/.style={
    scale only axis,
    anchor=north west,
    axis x line*=bottom,
    axis y line*=left,
    axis line style={draw=black!40,line width=.5pt},
    y axis line style={draw=none},
    y dir=reverse,
    enlarge x limits=false,
    enlarge y limits=false,
    scaled x ticks=false,
    tick align=outside,
    major tick length=2.5pt,
    tick style={draw=black,line width=.5pt},
    y tick style={draw=none},
    xticklabel style={font=\efficiencyTickFont,inner sep=1pt},
    yticklabel style={font=\efficiencyTaskFont,inner sep=1pt},
    xticklabel={\pgfmathprintnumber[fixed,precision=1,zerofill]{\tick}},
    clip=false,
  },
  efficiency intervals/.style={
    only marks,
    error bars/.cd,
    x dir=both,x explicit,
    error bar style={line width=.65pt},
    error mark options={rotate=90,mark size=1.15pt,line width=.55pt},
    /pgfplots/.cd,
  },
  efficiency packed/.style={
    efficiency intervals,color=packedgreen,
    mark=*,mark size=1.35pt,
    mark options={fill=packedgreen,draw=packedgreen,line width=.4pt},
  },
  efficiency quadratic/.style={
    efficiency intervals,color=quadorange,
    mark=square*,mark size=1.35pt,
    mark options={fill=quadorange,draw=quadorange,line width=.4pt},
  },
  efficiency native/.style={
    efficiency intervals,color=linearblue,
    mark=triangle*,mark size=1.8pt,
    mark options={fill=white,draw=linearblue,line width=.7pt},
  },
}
\tikzset{
  efficiency band/.style={fill=black!3.1,draw=none},
  efficiency grid/.style={draw=black!11,line width=.45pt},
  efficiency baseline/.style={draw=black!70,line width=.75pt,dash pattern=on 2.25pt off 1.5pt},
  efficiency separator/.style={draw=black!28,line width=.55pt},
}

\newcommand{\efficiencyPackedKey}{\tikz[baseline=-.5ex]\draw[packedgreen,mark=*,mark size=2pt] plot coordinates {(0,0)};}
\newcommand{\efficiencyQuadraticKey}{\tikz[baseline=-.5ex]\draw[quadorange,mark=square*,mark size=2pt] plot coordinates {(0,0)};}
\newcommand{\efficiencyNativeKey}{\tikz[baseline=-.5ex]\draw[linearblue,mark=triangle*,mark size=2.3pt,mark options={fill=white,line width=.7pt}] plot coordinates {(0,0)};}
\newcommand{\efficiencyLinearKey}{\tikz[baseline=-.5ex]\draw[efficiency baseline] (0pt,0pt)--(11pt,0pt);}

